The Atari Disk, a Metal-Poor Stellar Population in the Disk System of the Milky Way

We have developed a chemo-dynamical approach to assign 36,010 metal-poor SkyMapper stars to various Galactic stellar populations. Using two independent techniques (velocity and action space behavior), $Gaia$ EDR3 astrometry, and photometric metallicities, we selected stars with the characteristics of the "metal-weak" thick disk population by minimizing contamination by the canonical thick disk or other Galactic structures. This sample comprises 7,127 stars, spans a metallicity range of $-3.50<${\metal}~$<-0.8$, and has a systematic rotational velocity of $\langle V_\phi\rangle=154$\,km\,s$^{-1}$ that lags that of the thick disk. Orbital eccentricities have intermediate values between typical thick disk and halo values. The scale length is $h_{R}=2.48^{+0.05}_{-0.05}$\,kpc and the scale height is $h_{Z}=1.68^{+0.19}_{-0.15}$\,kpc. The metallicity distribution function is well fit by an exponential with a slope of $\Delta\log{\rm N}/\Delta\metal=1.13\pm0.06$. Overall, we find a significant metal-poor component consisting of 261 SkyMapper stars with \metal$<-2.0$. While our sample contains only eleven stars with {\metal}~$\lesssim-3.0$, investigating the JINAbase compilation of metal-poor stars reveals another 18 such stars (five have {\metal}$<-4.0$) that kinematically belong to our sample. These distinct spatial, kinematic and chemical characteristics strongly suggest this metal-poor, phase-mixed kinematic sample to represent an independent disk component with an accretion origin in which a massive dwarf galaxy radially plunged into the early Galactic disk. Going forward, we propose to call the metal-weak thick disk population as the Atari disk, given its likely accretion origin, and in reference to it sharing space with the Galactic thin and thick disks.

==> Atari Disk/tab1.tex <==
\begin{deluxetable*}{lrrrrrrrrrrr}
\caption{{Stellar Parameters and $Gaia$ Astrometric Solutions}}
\label{tab:Table_1}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{source\_id} & 
\colhead{parallax}&
\colhead{$\mu_{\alpha}$ $cos(\delta)$} &
\colhead{$\mu_{\delta}$} &  
\colhead{RV}           & 
\colhead{l}        &
\colhead{b}       &
\colhead{d$_{SDP}$}& 
\colhead{{\metal}}      & 
\colhead{{L$_z$}}    &  
\colhead{{J$_r$}} &
\colhead{{J$_z$}}\\
%
\colhead{}&
\colhead{(mas)}	  &
\colhead{(mas\,yr$^{-1}$)}&
\colhead{(mas\,yr$^{-1}$)}&
\colhead{(km\,s$^{-1}$)}	&
\colhead{(deg)}     &
\colhead{(deg)}	&	
\colhead{(kpc)}   &  
\colhead{(dex)}	  &	
\colhead{(kpc km\,s$^{-1}$)} &
\colhead{(kpc km\,s$^{-1}$)} &
\colhead{(kpc km\,s$^{-1}$)}
}
\startdata
2334983060942097664&0.671&2.330&$-$28.582&70.27&37.245&$-$78.457&1.49&$-$0.86&542.99&389.25&192.81\\
4918304837496677248&0.304&4.711&$-$0.954&53.08&314.997&$-$56.947&3.31&$-$0.79&1305.19&26.08&163.45\\
4901413310941027072&1.125&32.894&$-$1.159&119.69&312.286&$-$52.664&0.89&$-$1.12&1015.84&158.48&198.71\\
2421111311440455168&0.198&$-$2.679&$-$9.637&$-$104.37&80.127&$-$71.531&5.09&$-$3.20&607.15&696.21&236.33\\
2422492847800684416&0.300&$-$0.500&$-$23.563&$-$110.44&83.613&$-$70.002&3.36&$-$2.42&$-$607.64&753.16&219.27\\
2339756040919188480&0.257&5.320&$-$7.972&69.20&47.902&$-$77.903&3.93&$-$1.25&605.90&238.43&356.76\\
4991401092065999360&0.376&0.444&3.777&20.18&328.375&$-$68.950&2.67&$-$0.81&2081.24&131.16&145.21\\
2340071806914929920&0.517&$-$4.974&$-$34.741&$-$97.15&50.676&$-$77.698&1.96&$-$1.97&$-$215.55&884.75&90.11\\
4995919432020493440&0.475&$-$2.472&$-$1.622&$-$34.00&333.978&$-$71.668&2.11&$-$0.89&1867.50&54.88&102.31\\
2341853840385868288&0.320&5.335&$-$19.603&$-$110.72&62.991&$-$76.206&3.15&$-$1.74&$-$508.89&376.26&137.58\\
2314830593353777280&0.727&30.731&$-$7.730&$-$18.87&13.964&$-$78.469&1.38&$-$0.92&852.38&467.33&36.53\\
4994799132751744128&0.354&0.902&$-$4.096&$-$4.87&331.310&$-$70.548&2.84&$-$0.88&1411.96&37.25&127.50\\
4688252950170144640&0.437&22.078&$-$2.191&$-$28.16&307.226&$-$41.562&2.29&$-$1.06&1303.86&427.46&60.41\\
2320839596198507648&0.604&5.558&$-$11.909&9.12&14.965&$-$78.575&1.66&$-$1.05&1118.50&145.25&49.47\\
2340104929702744192&0.185&$-$1.568&$-$12.358&$-$59.60&51.845&$-$77.765&5.44&$-$1.34&$-$49.71&827.14&429.74\\
4901401907804117632&0.693&43.595&$-$24.514&7.91&312.082&$-$52.667&1.44&$-$1.39&$-$19.81&874.88&94.39\\
2340079091179498496&0.732&$-$12.163&$-$11.067&27.42&50.690&$-$77.917&1.38&$-$0.93&1792.91&178.37&47.83
\enddata
\tablecomments{Parallax is the corrected parallax based on \citet{Lindegren+2020b}. $d_{\text{SDP}}$ is the mean value of the 10,000 realizations and {\metal} adopted from \citet{Chiti2021}. The complete version of Table~\ref{tab:Table_1} is available online only. A short version is shown here to illustrate its form and content. Distance and actions are rounded to two digits, but are given at full numerical precision in the online table.}
\end{deluxetable*}





==> Atari Disk/tab2_properties.tex <==
\begin{table*}[ht!]
	\begin{center}
		\centering
		\caption{Orbital properties of the Galactic thin disk, thick disk, and inner halo}
		\label{tab:populations}
		\begin{tabular}{lccccr}
			\hline
			\hline	
			 Parameter & unit & Thin disk &  Thick disk & Inner halo & Atari disk\\
			\hline	
		     $h_{R}$&   (kpc)  &2.6\tablenotemark{a} - 3.0\tablenotemark{b}  & 2.0\tablenotemark{b} - 3.0\tablenotemark{c} & \nodata &  2.48 $\pm$ 0.05 \\
			 $h_{Z}$&   (kpc) &0.14\tablenotemark{d} - 0.36\tablenotemark{e}  & 0.5\tablenotemark{e} - 1.1\tablenotemark{e} & \nodata & 1.68$^{+0.19}_{-0.15}$ \\
			 $<V_{\phi}>$&   (km s$^{-1}$)               &  208\tablenotemark{e}  & 182\tablenotemark{g}&   0\tablenotemark{f}&  154 $\pm$ 1\\
		     Z$_{max}$&   (kpc)                         & $< 0.8$\tablenotemark{h}  & $0.8$ - $3.0$\tablenotemark{g} & $> 3.0$\tablenotemark{g} &  $<$ 3.0\\
		     e&  \nodata                                       & $< 0.14$\tablenotemark{g}  & 0.3 - 0.5\tablenotemark{g} & $>$ 0.7\tablenotemark{g}& 0.30 - 0.7\\
			\hline
		\end{tabular}
	\end{center}
	\tablenotetext{}{References are as follows: (a): \citealt{Juric2008}; (b): \citealt{Li2017}; (c): \citealt{Li2018}; (d): \citealt{Sanders2015}; (e): \citealt{Recio2014}; (f): \citealt{Carollo2010}; (g): \citealt{Lee2011}; (h):  \citealt{Anders2014}. }
\end{table*}





==> Atari Disk/tab3_hrz.tex <==
\begin{deluxetable}{lcccc}\label{tab:lengths_and_heights}
\tabletypesize{\scriptsize}
\tablecaption{Scale Lengths and Scale Heights for Different Metallicity Bins}
\tablehead{\colhead{Sample} &\colhead{Metallicity bin} & \colhead{$N_{\rm stars}$} &
  \colhead{scale length} & \colhead{scale height} \\
  & & & (kpc) & (kpc)}
\startdata
Common     &$-1.2\le {\rm [Fe/H]}<-0.8$ & 4,868 & \boldmath{$2.38^{+0.05}_{-0.05}$} & $1.75^{+0.17}_{-0.14}$\\
           &$-1.5\le {\rm [Fe/H]}<-1.2$ & 835   & \boldmath{$2.62^{+0.09}_{-0.09}$} & $1.36^{+0.31}_{-0.23}$\\
           &$-1.8\le {\rm [Fe/H]}<-1.5$ & 314   & \boldmath{$2.98^{+0.15}_{-0.15}$} & $1.41^{+1.37}_{-0.52}$\\
           &$-3.5\le {\rm [Fe/H]}<-1.8$ & 268   & \boldmath{$2.91^{+0.16}_{-0.16}$} & $2.03^{+2.82}_{-0.95}$\\
           &$-3.5\le {\rm [Fe/H]}<-0.8$ & 6,347 & \boldmath{$2.48^{+0.05}_{-0.05}$} & $1.67^{+0.20}_{-0.16}$\\
\hline
%----------------------------------------
Velocity   &$-1.2\le {\rm [Fe/H]}<-0.8$ & 5,570 & $2.64^{+0.04}_{-0.04}$ & $1.43^{+0.18}_{-0.15}$\\
           &$-1.5\le {\rm [Fe/H]}<-1.2$ & 993   & $3.30^{+0.10}_{-0.10}$ & $1.15^{+0.19}_{-0.16}$\\
           &$-1.8\le {\rm [Fe/H]}<-1.5$ & 414   & $4.00^{+0.11}_{-0.12}$ & $1.33^{+1.14}_{-0.48}$\\
           &$-3.5\le {\rm [Fe/H]}<-1.8$ & 394   & $4.14^{+0.09}_{-0.09}$ & $1.68^{+1.32}_{-0.56}$\\
           &$-3.5\le {\rm [Fe/H]}<-0.8$ & 7,451 & $3.00^{+0.05}_{-0.05}$ & $1.39^{+0.19}_{-0.16}$\\
\hline
%----------------------------------------
Action     &$-1.2\le {\rm [Fe/H]}<-0.8$ & 7,694 & $2.51^{+0.04}_{-0.04}$  & \boldmath{$1.92^{+0.17}_{-0.15}$}\\
           &$-1.5\le {\rm [Fe/H]}<-1.2$ & 1,497 & $2.95^{+0.08}_{-0.08}$  & \boldmath{$1.37^{+0.32}_{-0.22}$}\\
           &$-1.8\le {\rm [Fe/H]}<-1.5$ & 707   & $3.30^{+0.12}_{-0.12}$  & \boldmath{$1.63^{+1.19}_{-0.49}$}\\
           &$-3.5\le {\rm [Fe/H]}<-1.8$ & 639   & $3.38^{+0.12}_{-0.12}$  & \boldmath{$2.08^{+3.15}_{-1.10}$}\\
           &$-3.5\le {\rm [Fe/H]}<-0.8$ &10,351 & $2.70^{+0.04}_{-0.04}$  & \boldmath{$1.68^{+0.19}_{-0.15}$}\\
\hline
\hline
\multicolumn{4}{l}{Additional metallicity bins}\\
\hline
\hline
%----------------------------------------
Common     &$-0.9\le {\rm [Fe/H]}<-0.8$ & 1,960 & $2.32^{+0.06}_{-0.06}$ & $1.64^{+0.47}_{-0.30}$\\
           &$-1.1\le {\rm [Fe/H]}<-0.9$ & 2,161 & $2.41^{+0.06}_{-0.06}$ & $2.03^{+0.87}_{-0.48}$\\ %?
           &$-1.3\le {\rm [Fe/H]}<-0.8$ & 5,264 & $2.40^{+0.04}_{-0.05}$ & $1.73^{+0.18}_{-0.15}$\\ %?
           &$-3.5\le {\rm [Fe/H]}<-1.1$ & 1,964 & $2.73^{+0.07}_{-0.07}$ & $1.59^{+0.56}_{-0.34}$\\ %?
           &$-3.5\le {\rm [Fe/H]}<-1.3$ & 1,046 & $2.85^{+0.09}_{-0.08}$ & $1.52^{+0.59}_{-0.35}$\\ %?
           &$-3.5\le {\rm [Fe/H]}<-1.4$ & 786   & $2.92^{+0.10}_{-0.10}$ & $1.84^{+1.59}_{-0.60}$\\ %?
\hline
%----------------------------------------
Velocity   &$-0.9\le {\rm [Fe/H]}<-0.8$ & 2,231 & $2.51^{+0.07}_{-0.07}$ & $1.40^{+0.25}_{-0.20}$\\ %?
           &$-1.1\le {\rm [Fe/H]}<-0.9$ & 2,486 & $2.71^{+0.06}_{-0.06}$ & $1.64^{+0.58}_{-0.34}$\\ %?
           &$-1.3\le {\rm [Fe/H]}<-0.8$ & 6,040 & $2.70^{+0.05}_{-0.05}$ & $1.40^{+0.18}_{-0.15}$\\ %?
           &$-3.5\le {\rm [Fe/H]}<-1.1$ & 2,433 & $3.61^{+0.07}_{-0.07}$ & $1.30^{+0.36}_{-0.24}$\\ %?
           &$-3.5\le {\rm [Fe/H]}<-1.3$ & 1,369 & $3.96^{+0.09}_{-0.09}$ & $1.37^{+0.48}_{-0.30}$\\ %?
           &$-3.5\le {\rm [Fe/H]}<-1.4$ & 1,064 & $4.06^{+0.08}_{-0.08}$ & $1.61^{+0.97}_{-0.46}$\\ %?
\hline
%----------------------------------------
Action     &$-0.9\le {\rm [Fe/H]}<-0.8$ & 3,065 & $2.43^{+0.05}_{-0.05}$ & $1.65^{+0.28}_{-0.21}$\\ %?
           &$-1.1\le {\rm [Fe/H]}<-0.9$ & 3,422 & $2.53^{+0.06}_{-0.06}$ & $2.37^{+0.47}_{-0.35}$\\ %?
           &$-1.3\le {\rm [Fe/H]}<-0.8$ & 8,353 & $2.55^{+0.05}_{-0.05}$ & $1.80^{+0.17}_{-0.15}$\\ %?
           &$-3.5\le {\rm [Fe/H]}<-1.1$ & 3,760 & $3.09^{+0.06}_{-0.06}$ & $1.74^{+0.64}_{-0.37}$\\ %?
           &$-3.5\le {\rm [Fe/H]}<-1.3$ & 2,223 & $3.22^{+0.07}_{-0.07}$ & $1.83^{+0.77}_{-0.42}$\\ %?  
           &$-3.5\le {\rm [Fe/H]}<-1.4$ & 1,740 & $3.27^{+0.08}_{-0.08}$ & $2.14^{+2.25}_{-0.79}$\\ %?  
\hline
%----------------------------------------
Velocity (45)  &$-1.2\le {\rm [Fe/H]}<-0.8$ & 5,794 & $2.68^{+0.05}_{-0.04}$ & $1.49^{+0.24}_{-0.19}$\\
           &$-1.5\le {\rm [Fe/H]}<-1.2$     & 1,108 & $3.44^{+0.09}_{-0.10}$ & $1.44^{+0.36}_{-0.24}$\\
           &$-1.8\le {\rm [Fe/H]}<-1.5$     & 467   & $4.11^{+0.12}_{-0.12}$ & $1.26^{+1.43}_{-0.48}$\\
           &$-3.5\le {\rm [Fe/H]}<-1.8$     & 447   & $4.25^{+0.09}_{-0.10}$ & $2.82^{+4.61}_{-1.61}$\\
           &$-0.9\le {\rm [Fe/H]}<-0.8$     & 2,288 & $2.55^{+0.06}_{-0.06}$ & $1.39^{+0.20}_{-0.16}$\\
           &$-1.1\le {\rm [Fe/H]}<-0.9$     & 2,617 & $2.74^{+0.06}_{-0.06}$ & $1.71^{+0.54}_{-0.33}$\\
           &$-3.5\le {\rm [Fe/H]}<-1.1$     & 2,688 & $3.71^{+0.06}_{-0.07}$ & $1.65^{+0.58}_{-0.33}$\\
\hline
%----------------------------------------
\hline
Velocity (55)  &$-1.2\le {\rm [Fe/H]}<-0.8$ & 5,794 & $2.73^{+0.05}_{-0.05}$& $1.79^{+0.44}_{-0.29}$\\
           &$-1.5\le {\rm [Fe/H]}<-1.2$     & 1,108 & $3.56^{+0.10}_{-0.09}$ & $1.48^{+0.30}_{-0.22}$\\
           &$-1.8\le {\rm [Fe/H]}<-1.5$     & 467   & $4.34^{+0.10}_{-0.10}$ & $1.53^{+1.84}_{-0.61}$\\
           &$-3.5\le {\rm [Fe/H]}<-1.8$     & 447   & $4.42^{+0.10}_{-0.10}$ & $4.56^{+8.32}_{-4.56}$\\
           &$-0.9\le {\rm [Fe/H]}<-0.8$     & 2,386 & $2.59^{+0.06}_{-0.06}$ & $1.45^{+0.21}_{-0.17}$\\
           &$-1.1\le {\rm [Fe/H]}<-0.9$     & 2,647 & $2.79^{+0.06}_{-0.07}$ & $2.26^{+1.49}_{-0.63}$\\
           &$-3.5\le {\rm [Fe/H]}<-1.1$     & 2,821 & $3.88^{+0.07}_{-0.07}$ & $2.09^{+0.57}_{-0.36}$\\
\hline
\enddata
\tablecomments{We list results for various [Fe/H] bins for comparisons with other studies and sample sizes.}
\end{deluxetable}




==> Atari Disk/tab4.tex <==
\begin{deluxetable*}{lrlrrrrr}
\tiny
\caption{Very and extremely metal-poor SMSS stars with Atari disk kinematics}
\label{tab:SMSS_EMP}
\tablehead{
\colhead{R.A. (J2000)} & 
\colhead{Decl. (J2000)} & 
\colhead{Gaia ID} & 
\colhead{\metal$_{phot}$} & 
\colhead{\metal$_{lit}$} & 
\colhead{Z$_{max}$ [kpc]} &
\colhead{e}&
\colhead{References for \metal$_{lit}$} }
\startdata
% 11 41 08.86&$-$45 35 28.44&5378708937737332480&$-$2.50&$-$2.42&1.32&0.63&\citet{Bergemann2017}\\
% 19 10 10.55&$-$56 55 22.79&6637075256716056960&$-$2.50&\nodata&2.87&0.72&\\
% 17 48 10.23&$-$67 04 04.61&5812742011794490624&$-$2.51&\nodata&3.27&0.57&\\
% 19 42 03.65&$-$54 44 17.85&6641835940201642624&$-$2.51&\nodata&3.82&0.27&\\
% 20 54 23.47&$-$00 33 09.56&4227297165674750336&$-$2.52&$-$2.78&3.10&0.26&\cite{Hansen2018RPA}\\
% 19 46 04.55&$-$24 49 07.67&6767353163974393472&$-$2.52&\nodata&1.30&0.58&\\
% 18 13 45.67&$-$60 50 04.87&6634353175162138624&$-$2.52&\nodata&3.79&0.49&\\
% 01 49 07.95&$-$49 11 42.95&4941611597788129024&$-$2.53&$-$2.94&2.68&0.49&\cite{Hansen2018RPA}\\
% 18 55 44.29&$-$50 17 43.54&6660920571546685440&$-$2.54&\nodata&2.37&0.44&\\
% 21 09 58.05&$-$09 45 39.90&6896316222821807232&$-$2.56&$-$2.73&3.25&0.51&\cite{Hansen2018RPA}\\
% 20 33 22.75&$-$32 15 17.80&6793015215607699712&$-$2.56&$-$2.39&5.18&0.28&\cite{Buder+2021}\\
% 22 19 08.35&$-$23 33 46.88&6626606295405710848&$-$2.57&$-$2.44&2.84&0.45&\cite{Placco_rave_mrs+2018}\\
% 11 47 18.62&$-$27 34 24.91&3484273497118149504&$-$2.58&\nodata&2.27&0.42&\\
% 05 52 15.79&$-$39 53 18.61&4805034691496015104\tablenotemark{a}&$-$2.59&$-$2.05&1.34&0.69& \cite{Ruchti2011}\\
% 22 00 14.50&$-$12 27 07.72&2613316664213390464&$-$2.59&\nodata&2.52&0.48&\\
% 14 10 16.56&$-$22 07 00.92&6277121331901807488&$-$2.60&$-$2.25&3.07&0.40&\cite{Buder+2021}\\
% 00 45 23.80&$-$21 12 16.12&2350425495596387584&$-$2.60&$-$2.63&3.66&0.56&\cite{Ezzeddine2020_RPA}\\
% 20 05 50.15&$-$09 27 47.08&4191531774709865984&$-$2.61&\nodata&3.91&0.35&\\
% 21 35 34.67&$-$61 46 38.76&6403902139346451968&$-$2.61&$-$1.19&3.33&0.58& \cite{Buder+2021}\\
% 17 42 01.84&$-$49 37 56.20&5946667961218454016&$-$2.64&$-$1.87&1.89&0.44& \cite{Buder+2021}\\
% 05 20 41.73&$-$74 39 52.09&4649458920068852224&$-$2.64&\nodata&2.68&0.46&\\
% 20 53 26.12&$-$63 27 07.68&6450505523805659520&$-$2.66&$-$2.32&3.51&0.19& \cite{Buder+2021}\\
% 18 54 57.34&$-$43 47 02.53&6715023209426294144&$-$2.67&$-$2.43&1.79&0.43& \cite{Buder+2021}\\
% 20 39 30.03&$-$13 57 44.13&6899559747765150848&$-$2.68&\nodata&1.68&0.54&\\
% 18 12 10.46&$-$49 34 49.36&6706063838921970944&$-$2.68&$-$3.02&1.87&0.53& \cite{Hansen2018RPA}\\
% 23 37 04.91&$-$12 37 08.41&2432449097388072960&$-$2.69&\nodata&3.24&0.32&\\
% 23 13 00.03&$-$45 07 06.67&6529464133855343872&$-$2.71&$-$2.64&4.66&0.30& \cite{Hansen2018RPA}\\
% 12 42 15.72&$-$16 13 54.24&3523787024442853504&$-$2.72&\nodata&4.50&0.42&\\
% 13 54 24.64&$-$38 00 29.52&6115370840606774272&$-$2.72&$-$1.84&3.23&0.09& \cite{Buder+2021}\\
% 16 16 39.35&$-$32 33 26.71&6035641953958688896&$-$2.72&\nodata&1.29&0.43&\\
% 21 09 18.48&$-$36 35 47.14&6776164134760319488&$-$2.73&\nodata&4.88&0.41&\\
% 14 57 24.78&$-$22 17 09.18&6232023694256910720&$-$2.73&\nodata&3.83&0.33&\\
% 13 22 09.80&$-$43 54 10.30&6088604260826828160&$-$2.73&$-$2.52&2.33&0.20&\cite{Placco_rave_mrs+2018}\\
% 20 45 23.14&$-$25 32 05.01&6805351117598004096&$-$2.75&\nodata&3.74&0.06&\\
% 18 06 26.25&$-$56 41 12.72&6651865199939555456&$-$2.76&$-$2.39&2.36&0.67&\cite{Placco_rave_mrs+2018}\\
% 12 27 11.67&$-$17 58 19.81&3520145063974814464\tablenotemark{a}&$-$2.78&$-$2.73&1.74&0.63& \cite{Beers2017}\\
% 14 02 55.04&$-$47 39 00.57&6094382705528421504&$-$2.79&\nodata&2.20&0.18&\\
% 20 36 34.00&$-$43 25 05.15&6676351809220383872&$-$2.80&\nodata&3.32&0.62&\\
% 13 19 47.01&$-$04 23 10.18&3636133400286350976&$-$2.80&$-$2.89&4.79&0.31&\cite{Sakari2018_RPA}\\
% 20 39 03.65&$-$04 05 54.40&4224438989494243712&$-$2.81&\nodata&2.30&0.48&\\
% 13 39 06.19&$-$04 39 38.16&3633481073298252672&$-$2.81&\nodata&5.02&0.63&\\
% 09 36 07.34&$-$28 20 14.99&5633706540578910336&$-$2.82&\nodata&1.22&0.51&\\
% 11 14 47.77&$-$40 52 19.46&5395422480850056960\tablenotemark{a}&$-$2.83&$-$2.38&1.65&0.26& \cite{Bergemann2017}\\
% 10 27 31.57&$-$40 10 54.99&5440688962249489664&$-$2.84&\nodata&1.24&0.71&\\
% 10 56 41.52&$-$06 04 44.54&3764629274071203200&$-$2.87&\nodata&2.45&0.47&\\
% 19 00 04.73&$-$51 56 40.26&6657552909167911808&$-$2.87&\nodata&1.54&0.61&\\
% 11 09 27.77&$-$23 49 25.83&3536420000730863744&$-$2.87&$-$2.40&3.75&0.07& \cite{Buder+2021}\\
% 19 50 38.10&$-$49 59 33.32&6670128676486817536&$-$2.88&\nodata&2.43&0.34&\\
% 21 50 41.51&$-$10 50 58.33&6844345125675251328&$-$2.89&$-$2.98&5.20&0.36&\cite{Hollek2011}\\
% 14 35 31.93&$-$47 19 04.30&6097933372172416000&$-$2.90&\nodata&1.49&0.40&\\
% 04 06 58.71&$-$54 05 56.31&4779874227616110592&$-$2.92&$-$2.36&1.71&0.75&\cite{Placco_rave_mrs+2018}\\
% 02 33 42.27&$-$20 48 04.84&5127150298028227456\tablenotemark{a}&$-$2.92&$-$2.73&2.76&0.53&\cite{Beers2017}\\
% 22 02 16.36&$-$05 36 48.47&2668962496722780544&$-$2.92&$-$2.75&3.59&0.59&\cite{Hansen2018RPA}\\
% 12 56 35.10&$-$46 23 17.71&6134328310860149632&$-$2.96&$-$2.68&2.79&0.22&\cite{Placco_rave_mrs+2018}\\
% 18 40 59.86&$-$48 41 35.30&6704273765272548864&$-$2.96&$-$2.58&1.51&0.48&\cite{Ezzeddine2020_RPA}\\
12 35 57.41&$-$34 40 19.70&6158268802159564544&$-$3.00&\nodata& 4.10&0.45&\\
06 51 52.43&$-$25 07 02.22 & 2921777156667244032\tablenotemark{b} & $-$3.02 & \nodata & 0.89 & 0.21 &  \\
20 05 28.77&$-$54 31 25.97&6473118900280458240&$-$3.04&$-$3.01& 4.10&0.18&\cite{Best_and_Brightest}\\
16 23 29.34 &$-$65 17 53.33 & 5827787046034460672\tablenotemark{b} & $-$3.04 & $-$2.31 & 3.99 & 0.31 & \cite{Buder+2021}\\
09 29 49.73&$-$29 05 59.03&5633365176579363584&$-$3.10&$-$2.88& 0.90&0.45&\cite{Sakari2018_RPA}\\
19 25 0.04 & $-$15 57 43.35 & 4181010754108521472\tablenotemark{c} & $-$3.14 & \nodata & 1.49 & 0.28  & \\
18 11 39.41&$-$46 45 43.50&6707545022835614464&$-$3.24&\nodata& 1.90&0.42&\\
21 48 07.05&$-$43 43 23.74&6565897654232474240&$-$3.24&\nodata& 4.80&0.57&\\
14 59 14.59&$-$10 49 42.34&6313811313365806208&$-$3.31&\nodata& 3.70&0.41&\\
23 30 19.62&$-$08 13 15.20&2438343952886623744&$-$3.48&$-$3.20& 4.20&0.56&X. Ou et al 2022 (in prep)   \\
15 45 12.76 &$-$31 05 29.22 & 6016676026902257280\tablenotemark{b} & $-$3.53 & \nodata & 2.10 & 0.22 & \\
\enddata
\tablecomments{A short version is shown here to illustrate the table form and content, but the full content is accessible in the online table.}
% A short version is shown here to illustrate its form and content. Distance and actions are
% rounded to two digits, but are given at full numerical precision in the online table
% \tablenotetext{a}{Assigned as a thick disk star in the literature}
% \tablenotetext{b}{Action-selected sample star}
% \tablenotetext{c}{Velocity-selected sample star}
\end{deluxetable*}


==> Atari Disk/tab_jina.tex <==
\begin{deluxetable*}{lrlrrrrrr}
\caption{Very and extremely metal-poor stars with Atari disk kinematics from the literature (collected through JINAbase)}
\label{tab:jina30}
\tablehead{
\colhead{R.A. (J2000)} & 
\colhead{Decl. (J2000)} & 
\colhead{Simbad identifier} & 
\colhead{\metal$_{lit}$} & 
\colhead{\cfe} & 
\colhead{Z$_{max}$\,[kpc]} & 
\colhead{e} &
\colhead{Ref} }
\startdata
%
%
\hline\hline
16 28 56.15&$-$10 14 57.10&2MASS J16285613$-$1014576 &$-$2.00&0.24   &0.58&0.43&\cite{Sakari2018_RPA}\\
18 28 43.44&$-$84 41 34.81&2MASS J18284356$-$8441346 &$-$2.03&$-$0.39&3.19&0.32&\cite{Ezzeddine2020_RPA}\\
05 52 15.78&$-$39 53 18.47&TYC 7602-1143-1       &$-$2.05&\nodata&1.33&0.69&\cite{Ruchti2011}\\
00 25 50.30&$-$48 08 27.07&2MASS J00255030$-$4808270 &$-$2.06&0.27   &1.61&0.53&\cite{Barklem2005}\\
14 10 15.84&$-$03 43 55.20&2MASS J14101587$-$0343553 &$-$2.06&$-$0.09&1.17&0.71&\cite{Sakari2018_RPA}\\
02 21 55.60&$-$54 10 14.40&2MASS J02215557$-$5410143 &$-$2.09&0.00   &3.16&0.33&\cite{Holmbeck+2020_rpa}\\
23 05 50.54&$-$25 57 22.29&CD $-$26$^{\circ}$ 16470  &$-$2.13&\nodata&2.75&0.34&\cite{Ruchti2011}\\
13 43 26.70&$+$15 34 31.10&HD119516                 &$-$2.16&\nodata&1.07&0.52&\cite{For_2010}\\
15 54 27.29&$+$00 21 36.90&2MASS J15542729+0021368   &$-$2.18&0.42   &0.88&0.51&\cite{Sakari2018_RPA}\\
03 46 45.72&$-$30 51 13.32&HD23798                  &$-$2.22&\nodata&0.83&0.54&\cite{Roederer_2010}\\
15 02 38.50&$-$46 02 06.60&2MASS J15023852$-$4602066 &$-$2.23&$-$0.16&0.97&0.30&\cite{Holmbeck+2020_rpa}\\
04 01 49.00&$-$37 57 53.40&2MASS J04014897$-$3757533 &$-$2.28&$-$0.30&2.61&0.52&\cite{Holmbeck+2020_rpa}\\
23 02 15.75&$-$33 51 11.03&2MASS J23021574$-$3351110 &$-$2.29&   0.37&2.08&0.44&\cite{Barklem2005}\\
11 41 08.90&$-$45 35 28.00&2MASS J11410885$-$4535283 &$-$2.32&\nodata&1.33&0.63&\cite{Ruchti2011}\\
09 29 49.74&$-$29 05 59.20&2MASS J09294972$-$2905589 &$-$2.32&   0.11&0.92&0.46&\cite{Sakari2018_RPA}\\
19 16 18.20&$-$55 44 45.40&2MASS J19161821$-$5544454 &$-$2.35&$-$0.80&2.37&0.49&\cite{Hansen2018RPA}\\
22 49 23.56&$-$21 30 29.50&TYC 6393-564-1        &$-$2.38&\nodata&2.96&0.54&\cite{Ruchti2011}\\
00 31 16.91&$-$16 47 40.79&HD2796                   &$-$2.40&$-$0.48&1.13&0.68&\cite{Mardini_2019a}\\
11 58 01.28&$-$15 22 18.00&2MASS J11580127$-$1522179 &$-$2.41&   0.62&3.62&0.38&\cite{Sakari2018_RPA}\\
15 14 18.90&$+$07 27 02.80&2MASS J15141890+0727028   &$-$2.42&   0.47&3.66&0.55&\cite{Roederer_2010}\\
% 15 14 18.90&$+$07 27 02.81&BPS CS30306$-$0132       &$-$2.42&\nodata&3.38&0.54&\\
05 10 35.47&$-$15 51 38.30&UCAC4 371-007255        &$-$2.43&\nodata&0.74&0.60&\cite{Cohen_2013}\\
16 10 31.10&$+$10 03 05.60&2MASS J16103106+1003055   &$-$2.43&   0.53&2.49&0.23&\cite{Hansen2018RPA}\\
05 51 42.14&$-$33 27 33.76&TYC 7062-1120-1       &$-$2.46&\nodata&1.71&0.68&\cite{Holmbeck+2020_rpa}\\
23 16 30.80&$-$35 34 35.90&BPS CS30493$-$0071       &$-$2.46&$-$0.01&1.26&0.40&\cite{Roederer2014}\\
01 07 31.23&$-$21 46 06.50&UCAC4 342-001270        &$-$2.55&\nodata&3.28&0.11&\cite{Cohen_2013}\\
18 36 23.20&$-$64 28 12.50&2MASS J18362318$-$6428124 &$-$2.57&   0.10&1.37&0.24&\cite{Hansen2018RPA}\\
18 40 59.85&$-$48 41 35.30&2MASS J18405985$-$4841353 &$-$2.58&   0.60&1.50&0.48&\cite{Ezzeddine2020_RPA}\\
18 36 12.12&$-$73 33 44.17&2MASS J18361214$-$7333443 &$-$2.61&   0.10&2.13&0.48&\cite{Ezzeddine2020_RPA}\\
01 49 07.94&$-$49 11 43.16&CD $-$49$^{\circ}$ 506    &$-$2.65&\nodata&2.75&0.49&\cite{Ruchti2011}\\
09 47 19.20&$-$41 27 04.00&2MASS J09471921$-$4127042 &$-$2.67&$-$0.42&2.40&0.35&\cite{Holmbeck+2020_rpa}\\
21 51 45.74&$-$37 52 30.88&2MASS J21514574$-$3752308 &$-$2.76&   0.38&1.87&0.35&\cite{Beers_1992}\\
22 24 00.14&$-$42 35 16.05&2MASS J22240014$-$4235160 &$-$2.77&   0.14&2.45&0.49&\cite{Roederer2014}\\
15 56 28.74&$-$16 55 33.40&SMSS J155628.74$-$165533.4&$-$2.79&   0.36&2.15&0.36&\cite{Jacobson_2015}\\
22 02 16.36&$-$05 36 48.40&2MASS J22021636$-$0536483 &$-$2.80&$-$0.25&3.34&0.58&\cite{Hansen2018RPA}\\
03 01 00.70&$+$06 16 31.87&BPS CS31079$-$0028       &$-$2.84&\nodata&1.34&0.62&\cite{Roederer_2010}\\
04 19 45.54&$-$36 51 35.92&2MASS J04194553$-$3651359 &$-$2.89&   0.06&3.58&0.52&\cite{Roederer2014}\\
21 20 28.65&$-$20 46 22.90&BPS CS29506$-$0007       &$-$2.94&\nodata&1.02&0.45&\cite{Roederer2014}\\
14 35 58.50&$-$07 19 26.50&2MASS J14355850$-$0719265 &$-$2.99&$-$0.40&3.02&0.45&\cite{Ezzeddine2020_RPA}\\
20 42 48.77&$-$20 00 39.37&BD $-$20$^{\circ}$ 6008   &$-$3.05&$-$0.43&1.40&0.32&\cite{Roederer2014}\\
06 30 55.57&$+$25 52 43.81&SDSS J063055.57+255243.7\tablenotemark{a}&$-$3.05&\nodata&0.74&0.50&\cite{Aoki_2013}\\
13 03 29.48&$+$33 51 09.14&2MASS J12222802+3411318&$-$3.05&$-$0.18&3.93&0.61&\cite{Lai_2008}\\
00 20 16.20&$-$43 30 18.00&UCAC4 233-000355&$-$3.07&3.02&2.70&0.52&\cite{Cohen_2013}\\
13 19 47.00&$-$04 23 10.25&TYC 4961-1053-1\tablenotemark{a}&$-$3.10&$-$0.52&4.50&0.30&\cite{Hollek_2011}\\
12 45 02.68&$-$07 38 46.95&SDSS J124502.68$-$073847.0\tablenotemark{a}&$-$3.17&2.54&4.00&0.50&\cite{Aoki_2013}\\
14 16 04.71&$-$20 08 54.08&2MASS J14160471$-$208540&$-$3.20&1.44&1.92&0.54&\cite{Barklem2005}\\
13 22 35.36&$+$00 22 32.60&UCAC4 452-052732&$-$3.38&\nodata&2.98&0.45&\cite{Cohen_2013}\\
23 21 21.56&$-$16 05 05.65&HE 2318$-$1621\tablenotemark{a}&$-$3.67&0.54&3.64&0.58&\cite{Placco_2020}\\
11 18 35.88&$-$06 50 45.02&TYC 4928-1438-1\tablenotemark{a}&$-$3.73&0.08&4.71&0.31&\cite{Hollek_2011}\\
13 02 56.24&$+$01 41 52.12&UCAC4 459-050836&$-$3.88&1.34&2.80&0.26&\cite{Barklem2005}\\
09 47 50.70&$-$14 49 07.00&HE 0945$-$1435\tablenotemark{a}&$-$3.90&$<$2.03&0.76&0.57&\cite{Hansen_2015ApJ}\\
%
10 55 19.28&$+$23 22 34.02& SDSS J105519.28+232234.0\tablenotemark{a}&$-$4.00 & $<$0.70 & 2.20 & 0.45&\cite{Aguado_2017} \\
14 26 40.33&$-$02 54 27.49& HE 1424$-$0241\tablenotemark{a}&$-$4.05 & $<$0.63 & 3.50 & 0.41 &\cite{Cohen_2007ApJ} \\
12 47 19.47&$-$03 41 52.50& SDSS J124719.46$-$034152.4 &$-$4.11 & $<$1.61 & 1.71 & 0.24& \cite{Caffau2013} \\
12 04 41.39&$+$12 01 11.52& SDSS J120441.38+120111.5\tablenotemark{a}&$-$4.34 & $<$1.45 & 3.35 & 0.39& \cite{Placco2015ApJ} \\ 
10 29 15.15&$+$17 29 27.88& SDSS J102915.14+172927.9&$-$4.99 & $<$0.70 & 2.47 & 0.06&\cite{Caffau_2011C} \\
\enddata
\tablenotetext{a}{Stars that have too large uncertainties in their Gaia EDR3 astrometric data to be useful.
}
\end{deluxetable*} 
